Hop, Skip, and Overthink: Diagnosing Why Reasoning Models Fumble during Multi-Hop Analysis

The emergence of reasoning models and their integration into practical AI chat bots has led to breakthroughs in solving advanced math, deep search, and extractive question answering problems that requires a complex and multi-step thought process. Yet, a complete understanding of why these models hallucinate more than general purpose language models is missing. In this investigative study, we systematicallyexplore reasoning failures of contemporary language models on multi-hop question answering tasks. We introduce a novel, nuanced error categorization framework that examines failures across three critical dimensions: the diversity and uniqueness of source documents involved ("hops"), completeness in capturing relevant information ("coverage"), and cognitive inefficiency ("overthinking"). Through rigorous hu-man annotation, supported by complementary automated metrics, our exploration uncovers intricate error patterns often hidden by accuracy-centric evaluations. This investigative approach provides deeper insights into the cognitive limitations of current models and offers actionable guidance toward enhancing reasoning fidelity, transparency, and robustness in future language modeling efforts.

==> 1_introduction.tex <==

Language models (LMs) have demonstrated remarkable performance on multi-hop question answering (QA) benchmarks, such as HotpotQA \cite{hotpotqa}, where success requires sourcing knowledge from multiple documents. %Subsequent datasets, including MuSiQue \cite{musique} and 2WikiMultiHopQA \cite{ho2020constructingmultihopqadataset} address limitations in earlier benchmarks. 
MuSiQue \cite{musique} extends this task by posing harder questions that reduces shortcut reasoning and provides explicit reasoning paths to better assess multi-step inference.


% Despite impressive aggregate scores, these benchmarks and models often mask nuanced failures: models can exploit “disconnected reasoning” shortcuts (Trivedi et al., EMNLP 2020), answer overall questions correctly while failing individual hops (Tang et al., EACL 2021), or be misled by plausible but incorrect inference chains (Bhuiya et al., EMNLP 2024).

The traditional evaluation metrics employed in these tasks, such as the final answer accuracy or the F1 score, fail to distinguish between genuine multi-step inference, simple memorization (as exposed by counterfactual benchmarks such as CofCA; \cite{wu2025cofca}, and over-reliance on dataset artifacts. Moreover, emerging studies \cite{interpretinglanguagemodelscase, faithfulnessvsplausibilityunreliability} show that errors may stem from missing knowledge recall, misinterpretation of question intent, or retrieval failures in retrieval-augmented settings. 

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{hop.png}
    \caption{
\textbf{Illustration of Multi-hop Reasoning}
A language model answers via a three-hop reasoning chain. The back-and-forth between documents illustrates overthinking, where unnecessary steps are added beyond the ideal inference path.
}
    \label{fig:hop-transition}
\end{figure}

With these limitations in mind, we move beyond answer correctness and undertake an investigative exploration of reasoning failures in multi-hop QA to answer a central question: How and why do reasoning models break down when stitching together information across multiple sources? 
To address this,  we introduce a diagnostic framework that decomposes reasoning behavior along three core dimensions:
%(1) \textbf{Hops} refer to distinct pieces of retrieved information (e.g., entities or factual sentences) used to progress reasoning. They exclude comparisons, question interpretations, final conclusions, or repeated references to prior content;
(1) \textbf{Hops} A hop is a discrete step or transition in the reasoning process where the model moves from one piece of information (e.g., a fact, source, or knowledge base entry) to another in order to bridge connections and form a complete answer.
(2) \textbf{Coverage} evaluates whether all necessary reasoning steps are covered; and
(3) \textbf{Overthinking} refers to whether the model meanders into unnecessary or off-track reasoning.
These dimensions support both qualitative annotation and targeted quantitative evaluation of reasoning fidelity.

% To address this, we introduce a diagnostic framework that decomposes reasoning behavior along three orthogonal dimensions:
% \begin{enumerate}
% \item \textbf{Hops:} whether and how many distinct source documents the model leverages while reasoning;

% \item \textbf{Coverage:} the extent to which all necessary inference steps are executed without omission;

% \item \textbf{Overthinking:} instances where models perform superfluous or tangential reasoning that does not advance toward the correct answer.
% \end{enumerate}

In this paper, we introduce a detailed set of reasoning error categories and apply them to manually annotate model traces from six language models across three multi-hop QA datasets. Building on these annotations, we develop an automated evaluation framework that closely mirrors human judgments.

%scaled sub-question accuracy checks. Through this two-step approach, we uncover hidden reasoning pathologies, including shortcut exploitation, distractor confusion, and knowledge-recall lapses.

In this paper, we define seven fine-grained reasoning error categories and manually annotate up to 80 responses across three datasets and six models. To scale this analysis, we introduce an LLM-as-a-Judge framework that achieves 74\% hop match accuracy and 50–75\% label agreement with human annotations on 2Wiki, MuSiQue, and HotpotQA.

\paragraph{Contributions:}
We present a detailed analysis of multi-hop reasoning by curating and annotating model responses on three diverse datasets: 2WikiMultiHopQA, HotpotQA, and MuSiQue. Using a structured error taxonomy, we quantify the distribution of reasoning errors across models. Our study reveals common reasoning issues, such as breaking down in the middle of reasoning, adding unnecessary steps in complex cases, and providing correct answers despite flawed reasoning, especially on questions with many entities or confusing information. Finally, we evaluate the effectiveness of an LLM-as-a-Judge framework, which shows strong agreement with human annotations on simpler datasets while highlighting key limitations on more complex ones. This supports the use of scalable, semi-automated evaluation for reasoning analysis.

% \begin{itemize}
% \item
% We carefully curate and annotate model outputs on three diverse datasets: 2WikiMultiHopQA, HotpotQA, and MuSiQue, and quantify the distribution of reasoning errors using a structured error taxonomy.

% \item We uncover systematic reasoning pathologies, including mid-hop failure cascades, overthinking in complex contexts, and a disconnect between reasoning quality and answer correctness, especially on entity-dense or distractor-rich datasets.

% \item We evaluate the viability of LLM-as-a-Judge for reasoning analysis, showing strong agreement with human annotations on simpler datasets and outlining key limitations on harder ones. This supports scalable yet faithful evaluation of multi-hop reasoning.

% \item We identify comprehensive error patterns—such as disproportionate failure at mid-chain hops, over-reliance on memorized facts—that guide targeted remediation strategies (e.g., memory injections, stronger distractor training), etc.
% \item We also outline practical recommendations for dataset design, evaluation protocols, and model training aimed at enhancing faithfulness, transparency, and robustness in future multi-hop reasoning systems.

%\end{itemize}

==> 2_error_cats.tex <==
% {\color{blue}
% Q: Do humans have high agreement when annotating according to our definitions?

% Plot 1: (x-axis) -> Error category refinement; (y-axis): interannotator agreement;  [Reshmi]

%  (1) Error annotation guidelines; DONE
 
%  (2) How do we come to a good interannotator agreement --> error categories are good; 

%  (3) Setting up the eval pipeline at scale (human) and (auto-eval). 
% }

\subsection{Task Formalization}
We define \textbf{multi-hop QA} as the task of responding to complex questions, undertaken by reasoning models, that necessitate synthesizing information from multiple sources through a chain of reasoning steps. A \textbf{hop}, denoted by \( h_i \), refers to a distinct reasoning step wherein the model extracts supporting evidence from a \textbf{unique document} \( d_j \in D \). The number of hops in a reasoning path corresponds to the number of unique documents accessed, regardless of how much content is extracted from each. Figure~\ref{fig:hop-transition} illustrates this hop-based reasoning process, highlighting how models transition between documents.

For a question $Q$ and a collection of $m$ documents $D = \{d_1, d_2, \dots, d_m\}$, the task is to predict (1) an answer $A$ (a textual span within one of the documents in $D$), and (2) a reasoning path $\mathcal{P} = (h_1, h_2, \dots, h_{n_{\text{model}}})$ representing the sequence of reasoning hops.

The \textbf{model hop count} is defined as
\begin{equation}
N_{\text{model}} = |\mathcal{P}|,
\end{equation}
where $|\mathcal{P}|$ denotes the length of the model’s hop sequence.

The \textbf{gold hop count} is defined as
\begin{equation}
N_{\text{gold}} = |\mathcal{P}^*|,
\end{equation}
where $\mathcal{P}^*$ is the gold-standard reasoning path required to answer the question.


\subsection{Refining Reasoning Categories}
To diagnose reasoning failures in multi-hop QA, we refined our error taxonomy through three iterative stages. Each stage addressed prior shortcomings and improved inter-annotator agreement, as shown in Figure~\ref{fig:agreement-trend}. Full definitions for Stage 1 and Stage 2 are in the Appendix.

\subsubsection*{Stage 1: Coarse Conceptual Labels}
Our initial taxonomy used four loosely defined labels: \textit{Effective}, \textit{Underthinking}, \textit{Overthinking}, and \textit{Faulty}. These arose from manual trace inspection but lacked clear definitions. Annotators struggled to distinguish between concise reasoning and underthinking, or between verbose, incorrect reasoning and overthinking. The lack of a formal notion of reasoning hops made error tracing difficult. \textit{Faulty} served as a catch-all for various errors, reducing analytical usefulness.

\subsubsection*{Stage 2: Structured Hop-Based Categorization}
In the second stage, we introduced a 10-category taxonomy based on $N_{\text{model}}$, $N_{\text{gold}}$, hop correctness, and answer accuracy to support structured error analysis. As manual evaluation scaled, new ambiguities emerged. Category 8 (early hallucinations) often overlapped with Category 6 (underspecified chains) and question misinterpretation. Annotators also struggled to distinguish shortcut reasoning from flawed logic. These overlaps revealed that even structurally driven categories needed stronger semantic clarity.

\subsubsection*{Stage 3: Final Schema with Meta-Evaluation Markers}
The final schema addressed these issues through clearer definitions. We formally defined a reasoning \textbf{hop}, excluding repeated entity mentions within the same document to avoid inflated hop counts. We also distinguished overthinking via cross-document exploration ($N_{\text{model}}$ > $N_{\text{gold}}$) from verbose or circular reasoning within a document, captured by a separate overthinking flag.

These changes transformed the taxonomy into a more principled and disjoint framework. Annotator agreement improved significantly as category boundaries became more interpretable and semantically grounded.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Definitions of Reasoning Categories}
\label{sec:taxonomy}



\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\textwidth}{p{3.5cm} X}
\toprule
\textbf{Reasoning Category} & \textbf{Definition} \\
\midrule

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} = \bm{N}_{\text{gold}};$\\
\textit{Fully Correct Hops}
}
&
The model executes the exact number of required gold reasoning hops, and each hop is logically sound, complete, and correct. \\

\addlinespace

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} = \bm{N}_{\text{gold}};$\\
\textit{Partially Correct Hops}
}
&
The model executes the correct number of reasoning steps, but one or more hops involve incorrect documents, entities, or relations. The model reasoning is partially misaligned with the gold reasoning path. \\

\addlinespace

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} < \bm{N}_{\text{gold}};$\\
\textit{Fully Correct Hops}
}
&
The model executes fewer hops than required, yet all executed reasoning steps are correct and directly correspond to a subset of the required hops. This indicates incomplete but partially correct reasoning. \\

\addlinespace

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} < \bm{N}_{\text{gold}};$\\
\textit{Partially Correct Hops}
}
&
The model executes fewer reasoning steps than required, omitting essential hops and introducing incorrect hops within the shortened chain. The reasoning is both incomplete and partially incorrect. \\

\addlinespace

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} > \bm{N}_{\text{gold}};$\\
\textit{Trailing Irrelevance}
}
&
The model initially executes all required reasoning steps but then continues with additional irrelevant hops. These extra steps occur after completing the required reasoning and reflect the model's extraneous elaboration. \\

\addlinespace

\parbox[t]{3.5cm}{
$\bm{N}_{\text{model}} > \bm{N}_{\text{gold}};$\\
\textit{Early Irrelevance}
}
&
The model introduces irrelevant reasoning steps before or interspersed among the required hops. These interruptions disrupt logical reasoning progression, resulting in confusion, distraction or circular reasoning. The required reasoning steps may be partially addressed or incorrect. \\

\addlinespace

\parbox[t]{3.5cm}{
Question\\
Misinterpretation
}
&
The model misunderstands the original question during its early reasoning steps, often focusing on incorrect entities or setting up the wrong task, leading to fundamentally flawed reasoning. \\

\bottomrule
\end{tabularx}
\caption{Definitions of Reasoning Categories in Multi-Hop QA. $N_{\text{model}}$ denotes the number of reasoning hops executed by the model; $N_{\text{gold}}$ is the number of required gold hops.}
\label{tab:reasoning-categories}
\end{table*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.98\textwidth]{example.jpg} % Change to your filename/path
    \caption{
    \textbf{Examples of Reasoning Error Categories.}
    Representative outputs illustrating the main error categories in multi-hop reasoning for a single example. The correct entities are highlighted in green, incorrect in red, and irrelevant or extraneous information in yellow.
    }
    \label{fig:error-category-examples}
\end{figure*}

Following iterative refinement and extensive pilot annotations, we arrived at a final taxonomy that enabled high inter-annotator agreement. As shown in Figure~\ref{fig:agreement-trend}, this version resolved prior ambiguities by enforcing stricter hop semantics and introducing meta-evaluation markers to capture surface-level verbosity independently from structural reasoning failure.

Table~\ref{tab:reasoning-categories} summarizes our final taxonomy, providing precise operational definitions for each reasoning error category used in our annotation pipeline. These categories, combined with the meta-evaluation markers of overthinking and coverage, provide comprehensive coverage of potential reasoning errors, enabling systematic and insightful error diagnosis in multi-hop QA models.


\subsubsection*{Meta-Evaluation Markers}
To further enhance our analytical granularity, we introduced meta-evaluation markers:

\paragraph{Overthinking:} This marker captures indicators of cognitive inefficiency in the model's reasoning. It is applied when: 1) the model includes non-essential information from gold documents—such as background details, tangential facts, or calculations—that do not aid in progressing the reasoning chain; and 2) the model demonstrates repetitive or circular behavior, such as repeatedly checking the same entity or relation more than twice.

\paragraph{Coverage:} This marker addresses the completeness of source-document utilization, specifically evaluating whether the model successfully retrieves all necessary source documents. Low coverage indicates gaps in retrieval or attention, leading to incomplete reasoning chains or unsupported conclusions.


==> 3_experiments.tex <==


\paragraph{Models}
We analyze six language models that span a range of architectures, parameter scales, and accessibility. Our primary focus is on four open-source distilled models—\textsc{DeepSeek-R1-Distill-LLaMA-8B}, \textsc{DeepSeek-R1-Distill-LLaMA-70B}, \textsc{DeepSeek-R1-Distill-Qwen-7B}, and \textsc{DeepSeek-R1-Distill-Qwen-14B}. To complement these, we include two original reasoning models: \textsc{Claude 3.7 Sonnet}, a proprietary reasoning model, and \textsc{DeepSeek-R1}, an open-weight reasoning model.

For all DeepSeek models, we set the generation temperature to 0.6, following the recommendations of \citet{liu2024deepseek}, to mitigate endless repetition or incoherent outputs. For Claude 3.7 Sonnet, we use a deterministic setting with the temperature set to 0.

\paragraph{Datasets}
We evaluate model reasoning across three multi-hop QA datasets of increasing difficulty: 2WikiMultiHopQA~\cite{ho2020constructingmultihopqadataset}, which emphasizes structured multi-hop reasoning; HotpotQA~\cite{hotpotqa}, which includes distractors and diverse reasoning types like comparisons; and MuSiQue~\cite{musique}, a high-complexity benchmark designed to minimize shortcuts through dense context and sub-question dependencies. Dataset details are provided in Table~\ref{tab:dataset-stats} in the appendix.


% These datasets span a spectrum of reasoning difficulty, allowing us to assess model behavior in both constrained and artifact-resistant conditions. Table~\ref{tab:dataset-stats} summarizes their characteristics.



\subsubsection*{Question Types}

To enable systematic reasoning analysis, we categorize multi-hop questions into five distinct types based on their logical structure: \textit{Compositional}, \textit{Comparison}, \textit{Intersection}, \textit{Inference}, and \textit{Bridge Comparison}. These categories reflect the types of reasoning steps required to arrive at the correct answer.

Detailed definitions and illustrative examples for each type are provided in Appendix (Table~\ref{Appendix:question-types}).

\subsection{Annotation Process}
\label{sec:annotation}

To evaluate the reasoning quality of model outputs, we develop a structured human annotation pipeline encompassing three key stages:


    \paragraph{Sampling and Generation:}  
    We uniformly sampled 240 questions across HotpotQA, 2Wiki-MultiHopQA, and MuSiQue. Six models answered each question using a standardized prompting strategy designed to minimize instruction-induced bias. %and encourage faithful multi-hop reasoning grounded in the provided context.

    \paragraph{Final Answer and Meta Eval Markers:}  
    The final answers were evaluated for correctness using automated matching, with manual verification for paraphrased or non-exact responses. Simultaneously, we annotated: 1) the \(N_{\text{model}}\),  
    2) the binary \textit{Coverage} Marker and 3) the \textit{Overthinking Marker} .  

    \paragraph{Reasoning Category Assignment:}  
    Each response was categorized into one of our predefined reasoning error types. (see Section~\ref{sec:taxonomy}).

Figures~\ref{fig:interface1} and \ref{fig:interface2} show our custom annotation interface, which facilitates structured error labeling, flag toggling, and hop trace visualization.
In total, we annotated 1,440 model outputs. Following the removal of examples with missing answers in the context caused by dataset artifacts, 1,080 examples were retained for analysis.




\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{interann.png}
    \caption{
\textbf{Improvement in Inter-Annotator Agreement Across Refinement Stages.}
Raw agreement and Cohen’s kappa both increase substantially as the reasoning error taxonomy evolves from loosely defined to formally structured categories, with the highest agreement achieved after Stage 3 refinements.
}
    \label{fig:agreement-trend}
\end{figure}
 

==> 4_results.tex <==

% {\color{blue} 
% Q: What are the error patterns of different models (family, size)? How do they differ?

% (i) Quantitative Findings from the human-study - supported with some qualitative intuitions 
% - (Plot 2): (i) Non-reasoning Models; (ii) Reasoning Models;  [x-axis: error categories, y-axis: Reasoning accuracy] x [number of datasets]
% [Samyadeep / Ali]

% Q: Show examples and discuss why we think models make mistakes: e.g., distracted by extra details.
% - (Plot 3 / Table 0): Table showing some examples;  [Wenlong]
% }

% We analyze the reasoning behaviors of six language models across three multi-hop QA datasets—2WikiMultiHopQA, \textsc{HotpotQA}, and MuSiQue—focusing on reasoning correctness, overthinking, and answer accuracy. 

\subsection{Reasoning Fidelity and Answer Accuracy}

\begin{figure*}[htbp]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{2wiki_performance.png}
        \caption*{(a) 2Wiki}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{hotpot_performance.png}
        \caption*{(b) HotpotQA}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{musique_performance.png}
        \caption*{(c) MuSiQue}
    \end{minipage}
    \caption{
\textbf{Relationship Between Reasoning Fidelity and Answer Accuracy Across Datasets.}
Each subplot shows model performance on (a) 2Wiki, (b) HotpotQA, and (c) MuSiQue. Each point represents the performance of a model, with the x-axis showing the fraction of fully correct reasoning traces (\(N_{\text{model}}=N_{\text{gold}}\)) and the y-axis showing final answer accuracy. The dotted diagonal (\(y = x\)) marks perfect alignment; points above the line indicate models that answer correctly even when reasoning is imperfect.
}
    \label{fig:performance-trio}
\end{figure*}


\noindent Figure~\ref{fig:performance-trio} summarizes model behavior on fully correct hop alignment (\(N_{\text{model}}=N_{\text{gold}}\)) and final-answer accuracy across datasets.  We see that reasoning Fidelity holds in Simpler Tasks but collapses in Complex Chains. Across all datasets, Claude 3.7 achieves the highest accuracy.

% Across all three multi‑hop benchmarks we observe a positive—but decidedly loose—correlation between reasoning fidelity and final‑answer accuracy. In 2Wiki‑MultiHopQA and MuSiQue, markers trend upward, confirming that models which retrieve a larger fraction of fully correct reasoning chains also tend to answer more questions correctly. Yet the correlation is far from one‑to‑one: most points lie well above the implicit $y=x$ diagonal, indicating that models still achieve correct answers far more frequently than they produce perfectly faithful chains.
% Dataset‑level insights.
% 2Wiki‑MultiHopQA shows the steepest slope: markers cluster in the upper‑right corner, and the average gap between fidelity and accuracy is modest (≈ 0.10 – 0.15). This suggests the dataset effectively penalises shortcutting; when models improve fidelity they realise nearly proportional gains in accuracy. By contrast, MuSiQue exhibits a similar positive slope but with greater dispersion, implying higher variability in reasoning behaviour across models. (HotpotQA departs from this trend and is therefore discussed separately in the supplemental section.)
% Model‑level insights.
% Instruction‑tuned baselines—DeepSeek‑R1 and Claude‑3.7 Sonnet—excel at answer‑level heuristics: both deliver the highest answer accuracies while merely matching, or even trailing, their distilled counterparts on hop fidelity. This performance profile underscores a key risk of evaluating on answers alone: systems can “over‑perform” by exploiting dataset‑specific cues rather than constructing faithful multi‑hop chains.

\paragraph{High Reasoning Fidelity on 2Wiki:} All models perform strongly on the 2Wiki dataset, with the majority of models have around 80\% datapoints with \( N_{\text{model}} = N_{\text{gold}} \)correspondence: fully correct hops, and near-perfect final answer accuracy  This confirms that current LMs reliably handle simple multi-hop questions.

\paragraph{Inefficient Reasoning in HotpotQA: } Performance on HotpotQA shows the highest concentration of (\(N_{\text{model}}>N_{\text{gold}}\))
 (Figure~\ref{fig:reasoning-errors-hotpot}). While the final-answer accuracy remains high, the presence of semantically dense and distractor-filled paragraphs leads models to over-explore the context, often beyond the required inference chain. This behavior highlights the limitations of current LMs in maintaining focused reasoning under noisy, multi-document settings.


 \paragraph{Intermediate Fidelity and Model-Specific Patterns emerge on the MuSiQue dataset: } Larger models demonstrate intermediate reasoning fidelity (45–65\%) alongside relatively high answer accuracy. Smaller models exhibit poor performance on both metrics, underscoring difficulties in complex multi-hop contexts. Notably, DeepSeek-R1 shows the greatest divergence, achieving very high answer accuracy despite substantially lower reasoning fidelity.

 
 
% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{latex/images/reasoning_errors_musique.png}
%     \caption{Distribution of reasoning error types with Overthinking marker in MuSiQue across all models.}
%     \label{fig:reasoning-errors-musique}
% \end{figure*}


\subsection{Reasoning Patterns Across Models and Datasets}

Figure~\ref{fig:reasoning-errors-all} show the distribution of reasoning error types in the MuSiQue, 2Wiki-MultiHopQA, and HotpotQA datasets. Our analysis reveals the following insights:

\paragraph{Claude 3.7 Sonnet Sets the Bar for Stable and Precise Reasoning: }
Among all evaluated models, Claude 3.7 Sonnet demonstrates the most stable and controlled reasoning behavior. It consistently maintains high rates of fully correct reasoning while keeping all other error types—especially early and trailing irrelevance—significantly lower than both DeepSeek-R1 and the distilled model variants. %Claude shows minimal signs of misinterpretation or reasoning inefficiency, even in distractor-rich scenarios, highlighting its superior internal alignment and robustness across tasks.

% \paragraph{Reasoning Fidelity Holds in Simpler Tasks, Collapses in Complex Chains: }
% Models across families perform well on datasets like 2WikiMultiHopQA, consistently producing fully correct hop sequences with minimal errors (Figure ~\ref{fig:reasoning-errors-2wiki}). However, as reasoning complexity increases—as in HotpotQA and MuSiQue (Figure ~\ref{fig:reasoning-errors-hotpot} and Figure ~\ref{fig:reasoning-errors-mus}), the reasoning chain is derailed due to the presence of incorrect/inefficient reasoning. 

\paragraph{Overhopping is the Most Persistent and Systemic Reasoning Failure: }
Across all datasets and models, overhopping (\( N_{\text{model}} > N_{\text{gold}} \) categories in Figure ~\ref{fig:reasoning-errors-all}) is consistently higher than other errors. This often stems from contextual redundancy or ambiguity, pushing models to over-explore rather than terminate. The Qwen family of models particularly struggles with this issue: frequently displaying early and trailing irrelevance errors—even at larger scales—indicating a proclivity for recall over precise reasoning.

% \paragraph{Reasoning Performance Plateaus with Scale on Complex Tasks: }
% While scale brings early gains in accuracy, performance saturates on complex datasets such as those found in MuSiQue (Figure ~\ref{fig:reasoning-errors-mus}). Here, even large and reasoning-trained models fail to significantly outpace smaller distilled models, implying that architectural and training innovations beyond size are required to tackle deeper reasoning challenges.

% \paragraph{Model Scaling does not Always Reduce Errors: }
% Scaling consistently improves multi-hop accuracy and question comprehension. Larger models within both Qwen and LLaMA families see a drop in misinterpretation errors. However, trailing irrelevance remains common, suggesting that while scale mitigates early-stage errors, it does not guarantee improved reasoning control.


\paragraph{Scaling Models Improves Simple Reasoning but Leaves Complex Errors Unresolved:}
As shown in Figure~\ref{fig:reasoning-errors-all}, increasing model size leads to more examples with fully correct hops (the leftmost bars in each subplot), particularly on simpler tasks like 2Wiki (Figure~\ref{fig:reasoning-errors-all}a). However, for more complex datasets such as HotpotQA and MuSiQue (Figure~\ref{fig:reasoning-errors-all}b,~c), the gains from scaling plateau. Even the largest models still exhibit substantial numbers of early irrelevance and trailing irrelevance errors (the right-side bars). This persistent error pattern indicates that, while scale enhances basic multi-hop reasoning, it does not fully resolve deeper reasoning challenges in complex or distractor-heavy settings.

\paragraph{Deepseek-R1 Distilled Models Rival the Deepseek-R1 Counterpart in Multi-hop Tasks: }
%Distilled models such as \textsc{LLaMA-8B} and \textsc{70B} match or outperform explicitly reasoning-supervised models like \textsc{DeepSeek-R1}. 
On both simple and moderately complex datasets, distilled LLaMA variants show strong reasoning alignment. The LLaMA 70B variant performs almost similarly or even better than the original Deepseek-R1 model.



% \paragraph{Distilled Models vs Reasoning-Tuned Baselines.}
% Interestingly, distilled Llama models perform on par with or better than reasoning-tuned models like DeepSeek-R1. On 2Wiki, Llama-8B and 70B both achieve higher rates of fully correct hops, and even on more complex datasets like MuSiQue and HotpotQA, DeepSeek-R1 struggles with trailing irrelevance more than the Llama models. This suggests that distillation from high-quality teacher models and sufficient parameter scaling can rival explicit reasoning supervision in modeling multi-hop chains. Llama-70B, in particular, shows strong reasoning alignment and maintains coherent traces with only moderate elaboration errors in noisy contexts. Llama-8B, though smaller, achieves a solid balance between precision and coverage, with slightly more trailing irrelevance but minimal misinterpretation.



% \paragraph{Overall Trends.}
% Overall, we observe that scaling improves reasoning accuracy and question understanding, particularly in the Llama family. The Qwen models benefit from scaling but remain prone to overhopping. Distilled models, especially from the Llama family, effectively internalize reasoning structures and often outperform explicitly reasoning-trained counterparts. However, true reasoning control, especially in the presence of noisy or distractor-heavy contexts, remains a challenge for most models—except Claude Sonnet, which consistently maintains reasoning precision and efficiency across datasets.



\subsection{Relationship Between Reasoning Errors and Final Answer Correctness}

Figure~\ref{fig:answer-correctness-all} examines the relationship between reasoning trace quality and final answer correctness across datasets.

\paragraph{Correctness Tightly Coupled with Reasoning Quality:}
As seen in the leftmost bars in Figure~\ref{fig:answer-correctness-all}, across all datasets, final correct answers almost exclusively emerge from the (\( N_{\text{model}} = N_{\text{gold}} \)), Fully Correct Hops category. Even minor deviations in the reasoning chain, such as exceeding hops or partial hops, reduce the likelihood of correctness.

\paragraph{Answer Correctness is Sensitive to Missing Hops:}
Looking at the "Partially Correct Hops" bars in all three panels of Figure~\ref{fig:answer-correctness-all}, we see that incomplete reasoning rarely yields a correct answer. This confirms that failure to cover all necessary facts, even in part, is a definitive bottleneck in LMs’ reasoning chains.

\paragraph{Smaller Models are More Fragile to Reasoning Errors:}
As shown in Figure~\ref{fig:answer-correctness-all} across all datasets, smaller models such as LLaMA-8B and Qwen-7B exhibit a higher propensity for reasoning errors to cascade into incorrect final answers. In contrast, larger models like DeepSeek-R1 and Claude 3 Sonnet demonstrate greater robustness, with fewer incorrect answers arising from these types of reasoning errors.

\paragraph{Early Irrelevance is More Detrimental than Trailing Irrelevance:}
In every panel of Figure~\ref{fig:answer-correctness-all}, the "Early Irrelevance" category shows that "Answer Incorrect" bars are higher compared to that corresponding to "Trailing Irrelevance." This suggests that irrelevant reasoning steps introduced early in the chain are more disruptive%, whereas irrelevant steps at the end of the chain are less disruptive 
to the model’s final answer.

\begin{table*}[ht]
    \centering
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{2Wiki-MultiHopQA} & \textbf{HotpotQA} & \textbf{MuSiQue} \\
        \midrule
        DeepSeek-R1-Distill-Llama-8B      & 41.2\% & 29.3\% & 48.3\% \\
        DeepSeek-R1-Distill-Llama-70B     & 19.1\% & 12.0\% & 41.7\% \\
        DeepSeek-R1-Distill-Qwen-7B       & 26.5\% & 41.3\% & 61.7\% \\
        DeepSeek-R1-Distill-Qwen-14B      & 30.9\% & 28.0\% & 50.0\% \\
        DeepSeek-R1                       & 27.9\% & 18.7\% & 53.3\% \\
        Claude 3.7 Sonnet                 & 22.1\% & 22.7\% & 36.7\% \\
        \bottomrule
    \end{tabular}
    \caption{
\textbf{Overthinking Rates by Model and Dataset.}
Percentage of answers with Overthinking for each model on the 2Wiki-MultiHopQA, HotpotQA, and MuSiQue datasets. The results highlight the substantial increase in overthinking in more complex MuSiQue dataset.
}
\label{tab:overthinking-percentage}
\end{table*}



\subsection{Overthinking Trends and Their Impact}

We systematically examine the prevalence and impact of overthinking across different models and datasets, highlighting how this phenomenon influences overall model performance and error rates.


 \paragraph{Overthinking Surges in Complex Reasoning Tasks:} 
As shown in the MuSiQue results (see Figure~\ref{fig:reasoning-errors-all}c and Table~\ref{tab:overthinking-percentage}), overthinking rises markedly across all models, with rates ranging from 36.7\% to 61.7\%. Notably, DeepSeek-R1-Distill-Qwen-7B reaches the highest overthinking rate of 61.7\%, while even advanced models such as Claude 3 Sonnet and DeepSeek-R1 exhibit elevated rates. This trend suggests that task complexity, rather than model scale, is the primary driver of overthinking.

\paragraph{Overthinking is a Systematic Source of Incorrect Answers:} 
A significant portion of incorrect answers are accompanied by overthinking, especially in MuSiQue (see Figure~\ref{fig:answer-incorrectness-musique-overthink}). Although HotpotQA and 2Wiki contain fewer errors labeled as overthinking (see Table~\ref{tab:overthinking-percentage}), when overthinking does occur, it almost always results in incorrect answers (see shaded bars in Figure~\ref{fig:answer-incorrectness-2wiki-overthink} and Figure~\ref{fig:answer-incorrectness-hotpot-overthink}). This finding suggests that the negative impact of overthinking is not just limited to complex datasets but also arises from the logical incoherence it introduces, irrespective of task difficulty. Overthinking is not merely harmless elaboration, but a systematic driver of reasoning collapse and failure to reach a final answer.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{hopcomp.png}
    \caption{
\textbf{Hop-wise Distribution of Reasoning Errors in LLaMA Family Models.}
The left and right panels compare error trends for LLaMA-8B and LLaMA-70B, respectively. Results highlight the decline in fully correct reasoning with greater hop count, and the increasing prevalence of overhopping errors on harder questions.
}
\label{fig:hopwise-duo}
\end{figure*}

\subsection{Distribution across Question types}
Across the datasets, the multi-hop questions can be grouped into four key categories: \textit{Bridge Comparison questions}, \textit{Comparison questions}, \textit{Compositional questions}, and \textit{Inference Questions} (details of the question types and examples are in Section \ref{Appendix:question-types}).

Figure~\ref{fig:qtypes_error_all} shows the distribution of reasoning error types across question categories for all the models. We observe the following trends across different question types:


\paragraph{Bridge Comparison Questions Are Consistently Solved, Especially from 2Wiki:} Bridge questions (mainly from 2Wiki) yield 94–100\% fully correct hops across all models. Even smaller models like Qwen-7B and LLaMA-8B perform well, while Claude 3.7 Sonnet and Qwen-14B make no errors.  These questions often contain explicit reference to entities or co-occurrence patterns that mirror the pre-training distribution of the model, allowing models to resolve them through recognition of patterns at the surface level rather than deep reasoning.
    
\paragraph{Symmetric Structures Trigger Redundant Reasoning and Overhopping:} Found in HotpotQA and 2Wiki, comparison questions show 50–68\% fully correct rates, with 25–45\% of errors due to early or trailing irrelevance. Their symmetric phrasing encourages exploration of both options, even when one suffices. Claude occasionally bypasses intermediate hops while still producing correct answers, suggesting reliance on shortcut-style or selective reasoning paths.

\paragraph{Compositional Reasoning Exposes Integration Failures:} Compositional questions strain models’ ability to synthesize disjoint facts. Smaller models (Qwen-7B, LLaMA-8B, DeepSeek-R1) show many partially correct chains, even with correct hop counts. Claude and LLaMA-70B perform better, suggesting that scale and architecture improve integration. Misinterpretation errors are also higher here.

\paragraph{Inference Questions Are the Most Error-Prone and Trigger Overthinking:} Inference questions, heavily present in MuSiQue and 2Wiki, demand implicit reasoning and multi-step logic without strong lexical cues. These questions yield the broadest error types, early/trailing irrelevance, misinterpretation, and underhopping. Qwen-7B answers only 10\% correctly, with 30\% misinterpretation. Even DeepSeek-R1 shows 37\% trailing irrelevance. Only Claude and LLaMA-70B manage modest control (50–55\% correct), highlighting the inherent difficulty of inference.

\paragraph{Inference and Compositional Tasks Drive Overthinking:} Overhopping is most common in inference questions, reaching 70\% in Qwen-7B, 65\% in LLaMA-8B, and ~60\% in DeepSeek-R1 and Qwen-14B. Lack of clear stopping cues leads models to overgenerate. Bridge questions show minimal overhopping (<20\%) due to their bounded structure.

\paragraph{Even Large Models Struggle to Combine Retrieved Evidence:} In compositional and inference settings, all models — including large ones like DeepSeek-R1 and Claude 3.7 Sonnet — exhibit partially correct reasoning chains, even when hop counts match the gold labels. This reveals that accurate retrieval alone is insufficient; models must also effectively link and reason over retrieved evidence. These synthesis failures suggest weaknesses in chain-of-thought alignment and reasoning coordination, particularly under pressure from semantically distant facts.

% \vspace{-1em}  % adjust as needed
% \end{itemize}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{latex/images/llama8b_qtypes_w_errors.png}
%     \caption{Distribution of reasoning error types across different question types for DeepSeek-R1-Distill-LLaMA-8B.}

%     \label{fig:llama8b_qtypes}
% \end{figure}
%\vspace{-1em}  % adjust as needed

% Overall, these trends underscore that question complexity systematically amplifies error diversity, and that model scale alone does not eliminate failure modes like overthinking, shortcutting, or misinterpretation.



\subsection{Hop-wise Error Distribution}

To better understand how reasoning evolves across multi-hop inference chains, we analyze the distribution of reasoning errors at the hop level. Figure~\ref{fig:hopwise-duo} presents hop-wise error trends for the LLaMA family, while Figure~\ref{fig:hopwise_all} illustrates these trends for other models.


\paragraph{Larger Models Are More Stable Across Hop Counts:}
As the number of required reasoning steps increases, most models exhibit a clear drop in fully correct reasoning (\(N_{\text{model}} = N_{\text{gold}}\)). For example, in Figure~\ref{fig:hopwise-duo} (left panel), DeepSeek-R1-Distill-Llama-8B achieves 53\% accuracy on 2-hop questions, but this drops to 16\% for 3-hop and just 9\% for 4-hop examples. In contrast, larger models such as DeepSeek-R1-Distill-Llama-70B (Figure~\ref{fig:hopwise-duo}, right panel) and Claude 3.7 Sonnet (Figure~\ref{fig:hopwise_all}d) show much greater stability across hop lengths, maintaining relatively consistent performance even as reasoning depth increases. This suggests these models have a stronger capacity to follow and complete longer reasoning chains without deviation.

\paragraph{Overhopping Is a Major Error Source in Harder Questions:}
For 4-hop questions, the most prominent error across several models is early irrelevance (\(N_{\text{model}} > N_{\text{gold}}\)). This is especially clear for DeepSeek-R1-Distill-Qwen-7B (Figure~\ref{fig:hopwise_all}a), where 73\% of 4-hop examples are categorized as early irrelevance. Both Claude 3.7 Sonnet and DeepSeek-R1-Distill-Qwen-14B (Figure~\ref{fig:hopwise_all}b and d) show 45\% early irrelevance at 4 hops. These results indicate that, in more complex tasks, models frequently continue reasoning beyond what is necessary, retrieving irrelevant or redundant information.

\paragraph{Shallow Collapse in Qwen-7B, Depth Limitations in Claude 3.7 Sonnet: }
Qwen-7B (Figure~\ref{fig:hopwise_all}a) shows signs of partial reasoning at 3 hops but collapses almost entirely into early irrelevance (73\%) at 4 hops, abandoning intermediate reasoning strategies. This suggests that, under high reasoning load, smaller models tend to default to over-retrieval. In contrast, Claude 3.7 Sonnet (Figure~\ref{fig:hopwise_all}d) maintains strong performance up to 3 hops but shows a spike in early irrelevance (45\%) at 4 hops. Even advanced models, therefore, encounter depth calibration issues, struggling to determine when to stop in extended reasoning chains.



==> 5_autoeval.tex <==

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{autoeval3.png}
    \caption{
\textbf{Two-Step LLM-Assisted Evaluation Workflow.}
A high-level overview of the two-step decomposition that improves annotation accuracy and consistency for complex multi-hop reasoning tasks.
}
    \label{fig:autoeval}
\end{figure}


While extensive manual evaluations provide detailed and reliable insights into model reasoning behaviors, it is difficult to scale, particularly for complex queries from datasets like MuSiQue, where each annotation can take approximately four minutes per data point. Hence, We develop a framework for automating the annotation process to significantly improve evaluation efficiency.

\subsection{Evaluation Workflow}

We employed an LLM-as-a-Judge framework to automate the annotation task, using \texttt{gpt-4.1-mini}\footnote{%Note, the choice for utilizing GPT4.1-mini was done through a trial-and-error method.
A state-of-the-art model that is different from the models analyzed in this work.}
as our judging model. Utilizing LLM as a judge for annotating reasoning failures helped us scale the process significantly and reduced evaluation time, achieving approximately a \textbf{20x} increase in efficiency compared to manual annotation. To ensure parity with manual annotation process and high fidelity  analysis, we provided the Judge LLM with the same detailed annotation guidelines used by human annotators, but prompt-engineered the guidelines with explicit formatting instructions and clear definitions. The Judge LLM had access to 'question', 'relevant context documents', and the 'final response' from the reasoning models.

% Initially, we experimented with a single-step annotation approach, in which the Judge LLM received the entire annotation instruction set and input context simultaneously to directly categorize the responses. However, the performance of this single-step annotation was limited, primarily due to the cognitive overload associated with lengthy instructions and extensive context.

% To overcome these challenges, we adopted a two-step annotation process as illustrated Figure in \ref{fig:autoeval}:
% \begin{enumerate}

Consistent with findings for multi-step judging process in \cite{wang2023selfconsistencyimproveschainthought, zheng2024processbenchidentifyingprocesserrors}, we adopt a two-step annotation process as illustrated in Figure \ref{fig:autoeval}:


\begin{enumerate}

\item \textbf{Hop Breakdown}: First, the Judge LLM identifies and annotates the reasoning hops present in the model's response.

\item \textbf{Reasoning Classification}: Next, the Judge uses these annotated hops to accurately categorize the response into one of our predefined error categories.

\end{enumerate}
This decomposition significantly improved annotation accuracy and consistency, aligning with findings from recent literature indicating that multi-step judging processes enhance reliability and accuracy in complex evaluation tasks \cite{wang2022self}.

% The two-step LLM annotation process demonstrated substantial improvements over the single-step method. We observed enhanced consistency, reduced annotation errors, and overall higher agreement with manual annotations, validating the effectiveness of this automated, stepwise evaluation approach.

\subsection{Model-Wise Agreement with Human Annotations}

To further validate our LLM-as-a-Judge pipeline, we evaluate the consistency of annotations across six models and three datasets: \textsc{MuSiQue}, \textsc{2Wiki}, and \textsc{HotpotQA}. Based on the results presented in Table~\ref{tab:judge_model_agreement}, our LLM-as-a-Judge framework demonstrates promising potential for automating error categorization tasks traditionally performed by human annotators. Across all models and datasets, agreement rates vary, indicating model-specific and dataset-specific challenges. For example, models like DeepSeek-R1 and LLaMA 70B exhibit notably higher agreement rates, particularly on simpler datasets like \textsc{2Wiki}, achieving above 90\%. Conversely, the more challenging \textsc{MuSiQue} dataset consistently shows lower agreement scores, underscoring inherent complexities and subtle reasoning errors that the Judge LLM struggles to replicate accurately.

These results imply that while LLM-as-a-Judge systems are highly effective at automating error categorization for straightforward multi-hop reasoning tasks, complexities in certain datasets highlight the continuing necessity for human judgment or advanced refinement of Judge LLM instructions. The observed variability underscores that further investigation is essential to understand and mitigate factors contributing to lower Judge-model agreement rates, such as nuanced reasoning steps or subtle misinterpretations. Nonetheless, the substantial reduction in annotation time and generally high fidelity in simpler contexts strongly support the viability and efficiency of integrating LLM-as-a-Judge frameworks into broader NLP evaluation pipelines.

\begin{table}[h]
\centering
\caption{LLM-as-a-Judge Agreement (\%) with Human Annotations Across Models and Datasets}
\label{tab:judge_model_agreement}
\begin{tabular}{lrrr}
\toprule
      \textbf{Model} & \textbf{HotpotQA} & \textbf{2Wiki} & \textbf{MuSiQue} \\
\midrule
   LLaMA 8B    & 65.3 & 73.5 & 53.3 \\
   DeepSeek-R1 & 76.0 & 91.1 & 62.6 \\
   LLaMA 70B   & 72.0 & 92.6 & 75.0 \\
   Qwen 7B     & 66.6 & 75.0 & 46.6 \\
   Claude 3.7  & 73.3 & 91.1 & 76.6 \\
   Qwen 14B    & 65.3 & 88.2 & 78.3 \\
\bottomrule
\end{tabular}
\end{table}




% {\color{blue} 

% Q: Results for LLM-as-judge: Table (1) showing the correlations with human-agreement. Can LLM-as-a-judge work instead of humans for judging various error types?}
